Tell Me Who Your Friends Are: Using Content Sharing Behavior for News Source Veracity Detection

Stopping the malicious spread and production of false and misleading news has become a top priority for researchers. Due to this prevalence, many automated methods for detecting low quality information have been introduced. The majority of these methods have used article-level features, such as their writing style, to detect veracity. While writing style models have been shown to work well in lab-settings, there are concerns of generalizability and robustness. In this paper, we begin to address these concerns by proposing a novel and robust news veracity detection model that uses the content sharing behavior of news sources formulated as a network. We represent these content sharing networks (CSN) using a deep walk based method for embedding graphs that accounts for similarity in both the network space and the article text space. We show that state of the art writing style and CSN features make diverse mistakes when predicting, meaning that they both play different roles in the classification task. Moreover, we show that the addition of CSN features increases the accuracy of writing style models, boosting accuracy as much as 14\% when using Random Forests. Similarly, we show that the combination of hand-crafted article-level features and CSN features is robust to concept drift, performing consistently well over a 10-month time frame.

==> tex/labels_legend_table.tex <==
\newgeometry{left=2cm, top=1.4cm}

\begin{table*}[!ht]
    \fontsize{9}{9.2}\selectfont  % fontsize, spacing
    \renewcommand{\arraystretch}{1.4}
    \setlength{\tabcolsep}{2pt}
    \begin{tabular}[t]{L{3.6cm}lL{10.4cm}C{2.5cm}}
        \textbf{Section} & & \textbf{Description} \hfill (NewsGuard points) & \textbf{Coloring} \\ \hline
        %
        NewsGuard 
        & ~~1. & Does not repeatedly publish false content \hfill (22.0)  & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & ~~2. & Gathers and presents information responsibly \hfill (18.0) &  \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & ~~3. & Regularly corrects or clarifies errors \hfill (12.5)  &                                 \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~4. & Handles the difference between news and opinion responsibly \hfill (12.5)  &            \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~5. & Avoids deceptive headlines \hfill (10.0) &                                              \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~6. & Website discloses ownership and financing \hfill (7.5) &                               \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~7. & Clearly labels advertising \hfill (7.5) &                                              \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~8. & Reveals who's in charge, including any possible conflicts of interest \hfill (5.0) &   \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& ~~9. & Provides information about content creators \hfill (5.0) &                             \includegraphics[width=1.6ex]{fig/colors/green.pdf}
    	\includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
    	& 10. & Aggregated \texttt{score} computed from 1-9 & \includegraphics[width=1.6ex]{fig/colors/green.pdf} - \includegraphics[width=1.6ex]{fig/colors/purple.pdf} ~~ \\
    	& 11. & Column 10 thresholded at 60 points &
    	\includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/purple_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
    	% 
    	Pew Research Center 
    	& 12. & Trust from consistently-liberals & \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 13. & Trust from mostly-liberals & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 14. & Trust from mixed groups & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 15. & Trust from mostly-conservatives & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 16. & Trust from consistently-conservatives & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 17. & Aggregated trust from 12-16 & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
        % 
        Wikipedia 
        & 18. & Existence of source on Wikipedia's list of fake news sources & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\ \hline
        % 
        Open Sources 
        & 19. & Marked reliable & \includegraphics[width=1.6ex]{fig/colors/green.pdf} \\
        & 20. & Marked blog & \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 21. & Marked clickbait & \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 22. & Marked rumor & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 23. & Marked fake & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 24. & Marked unreliable & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 25. & Marked biased & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 26. & Marked conspiracy & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 27. & Marked hate speech & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 28. & Marked junk science & \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 29. & Marked political & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 30. & Marked satire & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 31. & Marked state news & \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\ \hline
        %
        Media Bias / Fact Check 
        & 32. & Factual reporting from 5 (good) down to 1 (bad) & 
        \includegraphics[width=1.6ex]{fig/colors/green.pdf}
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/purple_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 33. & Special label; conspiracy, pseudoscience or questionable source (purple), and satire (orange) &
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} 
        \includegraphics[width=1.6ex]{fig/colors/orange.pdf} \\
        & 34. & Political leaning / bias from left to right. & 
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/blue_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        Allsides 
        & 35. & Political leaning / bias & 
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/blue_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red_grey.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        BuzzFeed
        & 36. & Political leaning / bias, but only left and right &
        \includegraphics[width=1.6ex]{fig/colors/blue.pdf}
        \includegraphics[width=1.6ex]{fig/colors/red.pdf} \\ \hline
        %
        PolitiFact
        & 37. & Has brought story labelled as "pants on Fire!" &
        \includegraphics[width=1.6ex]{fig/colors/purple.pdf} \\
        & 38. & Has brought story labelled as false &
        \includegraphics[width=1.6ex]{fig/colors/purple2_grey.pdf} \\
        & 39. & Has brought story labelled as mostly false &
        \includegraphics[width=1.6ex]{fig/colors/purple_grey2.pdf} \\
        & 40. & Has brought story labelled as half-true &
        \includegraphics[width=1.6ex]{fig/colors/grey.pdf} \\
        & 41. & Has brought story labelled as mostly true &
        \includegraphics[width=1.6ex]{fig/colors/green_grey.pdf} \\
        & 42. & Has brought story labelled as true &
        \includegraphics[width=1.6ex]{fig/colors/green.pdf} \\ \hline
        %
        Alexa Ranking & & The Alexa ranking of the source. & Numerical \\ \hline
        %
        \# Articles & & The number of articles collected from the source. & Numerical \\ \hline
        %
        First Observed & & The date of first articles collected from the source. & dd-mm-yyyy \\ \hline
    \end{tabular}
    \caption{Details of the information for sources found in tables \ref{tab:source_labels1}, \ref{tab:source_labels2} and \ref{tab:source_no_labels}. We generally use green-to-purple for good-to-poor reliability/credibility, with grey as inconclusive. For bias we use blue-to-red for left-to-right bias, with grey as unbiased. Orange is used for special cases. In NewsGuard data it represents missing information, in Open Sources it marks auxiliary labels and for Media Bias / Fact Check it marks satire. }
    \label{tab:labelling_explanations}
\end{table*}

\restoregeometry

